A Quantum Internet Architecture

Entangled quantum communication is advancing rapidly, with laboratory and metropolitan testbeds under development, but to date there is no unifying Quantum Internet architecture. We propose a Quantum Internet architecture centered around the Quantum Recursive Network Architecture (QRNA), using RuleSet-based connections established using a two-pass connection setup. Scalability and internetworking (for both technological and administrative boundaries) are achieved using recursion in naming and connection control. In the near term, this architecture will support end-to-end, two-party entanglement on minimal hardware, and it will extend smoothly to multi-party entanglement and the use of quantum error correction on advanced hardware in the future. For a network internal gateway protocol, we recommend (but do not require) qDijkstra with seconds per Bell pair as link cost for routing; the external gateway protocol is designed to build recursively. The strength of our architecture is shown by assessing extensibility and demonstrating how robust protocol operation can be confirmed using the RuleSet paradigm.

==> acks.tex <==
%-------------------------------------------------------------------------------
\section*{Acknowledgments}
%-------------------------------------------------------------------------------

%Our work on quantum networking began in 2006; 
Over the years, a couple of dozen people have contributed to various elements of this architecture, some expressed in research papers, some in code or other artifacts, and some in discussion. Funding agencies are also to be thanked.

% Takaaki Matsuo, Clément Durand, Takahiko Satoh, Shota Nagayama, Shigeya Suzuki, Ryosuke Satoh, Sara Metwalli, Michal Hajdušek, Poramet Pathumsoot, Sujin Suwanna, Takafumi Oka, Luciano Aparicio, Kaori Ishizaki, Dominic Horsman, Joe Touch, Kae Nemoto, Bill Munro, Thaddeus Ladd, Austin Fowler, Simon Devitt, Andrew Greentree, Ashley Stephens, Liang Jiang, Wojciech Kozlowski, Angela Sara Cacciapuotti, Marcello Caleffi, and others


==> unused-text.tex <==

%%  LocalWords:  endnotes includegraphics fread ptr nobj noindent
%%  LocalWords:  pdflatex acks
%-------------------------------------------------------------------------------
\section{Footnotes, Verbatim, and Citations}
%-------------------------------------------------------------------------------

Footnotes should be places after punctuation characters, without any
spaces between said characters and footnotes, like so.%
\footnote{Remember that USENIX format stopped using endnotes and is
  now using regular footnotes.} And some embedded literal code may
look as follows.

\begin{verbatim}
int main(int argc, char *argv[]) 
{
    return 0;
}
\end{verbatim}

Now we're going to cite somebody. Watch for the cite tag. Here it
comes. Arpachi-Dusseau and Arpachi-Dusseau co-authored an excellent OS
book, which is also really funny~\cite{arpachiDusseau18:osbook}, and
Waldspurger got into the SIGOPS hall-of-fame due to his seminal paper
about resource management in the ESX hypervisor~\cite{waldspurger02}.

The tilde character (\~{}) in the tex source means a non-breaking
space. This way, your reference will always be attached to the word
that preceded it, instead of going to the next line.

And the 'cite' package sorts your citations by their numerical order
of the corresponding references at the end of the paper, ridding you
from the need to notice that, e.g, ``Waldspurger'' appears after
``Arpachi-Dusseau'' when sorting references
alphabetically~\cite{waldspurger02,arpachiDusseau18:osbook}. 

It'd be nice and thoughtful of you to include a suitable link in each
and every bibtex entry that you use in your submission, to allow
reviewers (and other readers) to easily get to the cited work, as is
done in all entries found in the References section of this document.

Now we're going take a look at Section~\ref{sec:figs}, but not before
observing that refs to sections and citations and such are colored and
clickable in the PDF because of the packages we've included.

%-------------------------------------------------------------------------------
\section{Floating Figures and Lists}
\label{sec:figs}
%-------------------------------------------------------------------------------


Here's a typical reference to a floating figure:
Figure~\ref{fig:vectors}. Floats should usually be placed where latex
wants then. Figure\ref{fig:vectors} is centered, and has a caption
that instructs you to make sure that the size of the text within the
figures that you use is as big as (or bigger than) the size of the
text in the caption of the figures. Please do. Really.

In our case, we've explicitly drawn the figure inlined in latex, to
allow this tex file to cleanly compile. But usually, your figures will
reside in some file.pdf, and you'd include them in your document
with, say, \textbackslash{}includegraphics.

Lists are sometimes quite handy. If you want to itemize things, feel
free:

\noindent
The noindent at the start of this paragraph in its tex version makes
it clear that it's a continuation of the preceding paragraph, as
opposed to a new paragraph in its own right.

\begin{figure*}
\includegraphics[width=14cm]{1D-interference-app.png}
\caption{JavaScript app allowing the learner to adjust various
  parameters to learn about one-dimensional interference.
  Constructive and destructive interference are the key to quantum
  algorithms.}
\label{fig:kiki}
\end{figure*}

\begin{figure*}
\includegraphics[width=14cm]{2D-interference-app.png}
\caption{JavaScript app for understanding two-dimensional
  interference, created using the D3 library.}
\label{fig:hideo}
\end{figure*}

\begin{figure*}[h]
\begin{center}
\includegraphics[width=10cm]{teleportation-overview-v3}
\caption{Operations in teleporting a qubit from Alice to Bob.}
\label{fig:teleport}
\end{center}
\end{figure*}

% inlined bib file
\usepackage{filecontents}

%-------------------------------------------------------------------------------


